Approximating Aggregated SQL Queries With LSTM Networks

Despite continuous investments in data technologies, the latency of querying data still poses a significant challenge. Modern analytic solutions require near real-time responsiveness both to make them interactive and to support automated processing. Current technologies (Hadoop, Spark, Dataflow) scan the dataset to execute queries. They focus on providing a scalable data storage to maximize task execution speed. We argue that these solutions fail to offer an adequate level of interactivity since they depend on continual access to data. In this paper we present a method for query approximation, also known as approximate query processing (AQP), that reduce the need to scan data during inference (query calculation), thus enabling a rapid query processing tool. We use LSTM network to learn the relationship between queries and their results, and to provide a rapid inference layer for predicting query results. Our method (referred as ``Hunch``) produces a lightweight LSTM network which provides a high query throughput. We evaluated our method using twelve datasets and compared to state-of-the-art AQP engines (VerdictDB, BlinkDB) from query latency, model weight and accuracy perspectives. The results show that our method predicted queries' results with a normalized root mean squared error (NRMSE) ranging from approximately 1\% to 4\% which in the majority of our data sets was better then the compared benchmarks. Moreover, our method was able to predict up to 120,000 queries in a second (streamed together), and with a single query latency of no more than 2ms.

==> comparison_table.tex <==
\begin{comment}
\begin{tabular}
{|p{0.7in}|p{0.4in}|p{0.5in}|p{0.5in}|p{0.7in}|p{0.5in}|p{0.6in}|p{0.5in}|} \hline\centering 
\newline \newline Attributes & Bagchi et al\newline (2007) & Babcock et al\newline (2002) & Chuang el al\newline (2009) & Chandramo\newline uli et al  (2011) & Zaharia et al\newline (2016) & Ramnara\newline yan et al (2016) & Our method \\ \hline \centering
Sampling & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}  \\ \hline\centering 
Recent data prioritization & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \\ \hline \centering
Predefined summaries \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \\ \hline 
User queries generation & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \\ \hline 
Distributed processing & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & NA & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \\ \hline 
Persist data & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \\ \hline 
Access data during querying & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \\ \hline \centering
Model/\newline Method footprint \centering& Mb \centering& Data dependent\centering & \centering Data dependent & Data dependent \centering& Data dependent \centering& Data dependent \centering& Mb \\ \hline \centering
Queries throughput (queries per second) \centering& NA \centering& NA \centering& NA \centering& $\mathrm{>}$1M (distributed computing) \centering& 10-100 \centering& NA & 10k-30k (single gpu) \\ \hline \centering
Real-time data query & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png} \centering& \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/vi.png}\centering & \includegraphics*[width=0.20in, height=0.20in, keepaspectratio=false]{Figures/x.png} \\ \hline 
\end{tabular}
\end{comment}

